Adaptive Pricing for Optimal Coordination in Networked Energy Systems with Nonsmooth Cost Functions

Incentive-based coordination mechanisms for distributed energy consumption have shown promise in aligning individual user objectives with social welfare, especially under privacy constraints. Our prior work proposed a two-timescale adaptive pricing framework, where users respond to prices by minimizing their local cost, and the system operator iteratively updates the prices based on aggregate user responses. A key assumption was that the system cost need to smoothly depend on the aggregate of the user demands. In this paper, we relax this assumption by considering the more realistic model of where the cost are determined by solving a DCOPF problem with constraints. We present a generalization of the pricing update rule that leverages the generalized gradients of the system cost function, which may be nonsmooth due to the structure of DCOPF. We prove that the resulting dynamic system converges to a unique equilibrium, which solves the social welfare optimization problem. Our theoretical results provide guarantees on convergence and stability using tools from nonsmooth analysis and Lyapunov theory. Numerical simulations on networked energy systems illustrate the effectiveness and robustness of the proposed scheme.

==> main <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{ruiz2009direct}
N.~Ruiz, I.~Cobelo, and J.~Oyarzabal, ``A direct load control model for virtual power plant management,'' \emph{IEEE Transactions on Power Systems}, vol.~24, no.~2, pp. 959--966, 2009.

\bibitem{chen2014distributed}
C.~Chen, J.~Wang, and S.~Kishore, ``A distributed direct load control approach for large-scale residential demand response,'' \emph{IEEE Transactions on Power Systems}, vol.~29, no.~5, pp. 2219--2228, 2014.

\bibitem{rahimi2010demand}
F.~Rahimi and A.~Ipakchi, ``Demand response as a market resource under the smart grid paradigm,'' \emph{IEEE Transactions on smart grid}, vol.~1, no.~1, pp. 82--88, 2010.

\bibitem{peplinski2023residential}
M.~Peplinski and K.~T. Sanders, ``Residential electricity demand on caiso flex alert days: a case study of voluntary emergency demand response programs,'' \emph{Environmental Research: Energy}, vol.~1, no.~1, 2023.

\bibitem{vardakas2014survey}
J.~S. Vardakas, N.~Zorba, and C.~V. Verikoukis, ``A survey on demand response programs in smart grids: Pricing methods and optimization algorithms,'' \emph{IEEE Communications Surveys \& Tutorials}, vol.~17, no.~1, pp. 152--178, 2014.

\bibitem{li2017distributed}
P.~Li, H.~Wang, and B.~Zhang, ``A distributed online pricing strategy for demand response programs,'' \emph{IEEE Transactions on Smart Grid}, vol.~10, no.~1, pp. 350--360, 2017.

\bibitem{khezeli2017risk}
K.~Khezeli and E.~Bitar, ``Risk-sensitive learning and pricing for demand response,'' \emph{IEEE Transactions on Smart Grid}, vol.~9, no.~6, pp. 6000--6007, 2017.

\bibitem{kong2020online}
X.~Kong, D.~Kong, J.~Yao, L.~Bai, and J.~Xiao, ``Online pricing of demand response based on long short-term memory and reinforcement learning,'' \emph{Applied energy}, vol. 271, p. 114945, 2020.

\bibitem{LI2024EPSR}
J.~Li, M.~Motoki, and B.~Zhang, ``Socially optimal energy usage via adaptive pricing,'' \emph{Electric Power Systems Research}, vol. 235, p. 110640, Oct. 2024.

\bibitem{maheshwari2022inducing}
C.~Maheshwari, K.~Kulkarni, M.~Wu, and S.~S. Sastry, ``Inducing social optimality in games via adaptive incentive design,'' in \emph{Conference on Decision and Control (CDC)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2022, pp. 2864--2869.

\bibitem{stott2009dc}
B.~Stott, J.~Jardim, and O.~Alsa{\c{c}}, ``Dc power flow revisited,'' \emph{IEEE Transactions on Power Systems}, vol.~24, no.~3, pp. 1290--1300, 2009.

\bibitem{zhang2021convex}
L.~Zhang, Y.~Chen, and B.~Zhang, ``A convex neural network solver for dcopf with generalization guarantees,'' \emph{IEEE Transactions on Control of Network Systems}, vol.~9, no.~2, pp. 719--730, 2021.

\bibitem{Bertsimas1997linear}
D.~Bertsimas and J.~N. Tsitsiklis, \emph{Introduction to linear optimization}.\hskip 1em plus 0.5em minus 0.4em\relax Belmont, Mass. : Athena Scientific, 1997.

\bibitem{Mallada2017tac}
E.~Mallada, C.~Zhao, and S.~Low, ``Optimal load-side control for frequency regulation in smart grids,'' \emph{IEEE Transactions on Automatic Control}, vol.~62, no.~12, pp. 6294--6309, Dec. 2017.

\bibitem{DORFLER2017Auto}
F.~D{\"o}rfler and S.~Grammatico, ``Gather-and-broadcast frequency control in power systems,'' \emph{Automatica}, vol.~79, pp. 296--305, May 2017.

\bibitem{WSU1972AM}
{Mathematics Department at Wayne State University}, ``Every convex function is locally lipschitz,'' \emph{The American Mathematical Monthly}, vol.~79, no.~10, p. 1121–1124, Dec. 1972.

\bibitem{Bertsekas2009Convex}
D.~P. Bertsekas, \emph{Convex Optimization Theory}.\hskip 1em plus 0.5em minus 0.4em\relax Athena Scientific, 2009.

\bibitem{Wright2022Optimization}
S.~J. Wright and B.~Recht, \emph{Optimization for Data Analysis}.\hskip 1em plus 0.5em minus 0.4em\relax Cambridge University Press, 2022.

\bibitem{Clarke1998Nonsmooth}
F.~H. Clarke, Y.~S. Ledyaev, R.~J. Stern, and P.~R. Wolenski, \emph{Nonsmooth Analysis and Control Theory}.\hskip 1em plus 0.5em minus 0.4em\relax Springer-Verlag, 1998.

\bibitem{Boyd2004convex}
S.~Boyd and L.~Vandenberghe, \emph{Convex optimization}.\hskip 1em plus 0.5em minus 0.4em\relax Cambridge university press, 2004.

\bibitem{Rudin2013PMA}
W.~Rudin, \emph{Principles of Mathematical Analysis}, 3rd~ed.\hskip 1em plus 0.5em minus 0.4em\relax McGraw Hill, 2013.

\bibitem{rockafellar1998}
R.~T. Rockafellar and R.~J.~B. Wets, \emph{{Variational Analysis}}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 1998.

\bibitem{Cortes2008CSM}
J.~Cortes, ``Discontinuous dynamical systems,'' \emph{IEEE Control Systems Magazine}, vol.~28, no.~3, pp. 36--73, June 2008.

\bibitem{Lax2017MultiCal}
P.~D. Lax and M.~S. Terrell, \emph{Multivariable Calculus with Applications}, 1st~ed.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2017.

\bibitem{Hirsch2013Hirsch}
M.~W. Hirsch, S.~Smale, and R.~L. Devaney, \emph{Differential Equations, Dynamical Systems, and an Introduction to Chaos}, 3rd~ed.\hskip 1em plus 0.5em minus 0.4em\relax Elsevier, 2013.

\bibitem{Spivak1965Calculus}
M.~Spivak, \emph{Calculus on Manifolds: A Modern Approach to Classical Theorems of Advanced Calculus}.\hskip 1em plus 0.5em minus 0.4em\relax Addison-Wesley Publishing Company, 1965.

\bibitem{Clason2024Nonsmooth}
C.~Clason, \emph{Nonsmooth Analysis and Optimization}.\hskip 1em plus 0.5em minus 0.4em\relax University of Graz, 2024.

\bibitem{Shevitz1994tac}
D.~Shevitz and B.~Paden, ``Lyapunov stability theory of nonsmooth systems,'' \emph{IEEE Transactions on Automatic Control}, vol.~39, no.~9, pp. 1910--1914, Sept. 1994.

\bibitem{zhang2014network}
B.~Zhang, R.~Rajagopal, and D.~Tse, ``Network risk limiting dispatch: Optimal control and price of uncertainty,'' \emph{IEEE Transactions on Automatic Control}, vol.~59, no.~9, pp. 2442--2456, 2014.

\end{thebibliography}

